Generalization of Graph Neural Networks through the Lens of Homomorphism

Despite the celebrated popularity of Graph Neural Networks (GNNs) across numerous applications, the ability of GNNs to generalize remains less explored. In this work, we propose to study the generalization of GNNs through a novel perspective - analyzing the entropy of graph homomorphism. By linking graph homomorphism with information-theoretic measures, we derive generalization bounds for both graph and node classifications. These bounds are capable of capturing subtleties inherent in various graph structures, including but not limited to paths, cycles and cliques. This enables a data-dependent generalization analysis with robust theoretical guarantees. To shed light on the generality of of our proposed bounds, we present a unifying framework that can characterize a broad spectrum of GNN models through the lens of graph homomorphism. We validate the practical applicability of our theoretical findings by showing the alignment between the proposed bounds and the empirically observed generalization gaps over both real-world and synthetic datasets.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/removed_contents.tex <==

\subsection{Impact of $F$ on Expressivity}
\label{sec:expressivity}

Before we introduced the isomorphism completeness of homomorphism representations given $\mathcal{F}$ contains all graphs up to size $V_G$. It is known that completeness is achievable with smaller classes of graphs such as 2-degenerated graphs and graphs homomorphic to non-bipartite graphs~\cite{Dvorak2010-rv}. We hereby discuss how $F$ can be reduced without degrading completeness.

We define $F_1F_2$ as the (gluing) product of $F_1$ and $F_2$ by taking their disjoint union. 
\begin{lemma}
For any graphs $G$, $F_1$ and $F_2$, $\hom(F_1F_2,G) = \hom(F_1, G)\hom(F_2, G)$~\cite{lovasz2012}.
\end{lemma}
This implies we only need connected graphs in $\mathcal{F}$ to be isomorphism complete. As homomorphism numbers and vice versa govern subgraph numbers,  this coincides with the findings from \citet{Wang_undated-iz} that connected subgraph counts infer disconnected subgraph counts.


% \cite{Barcelo2021-rs} extends this to rooted homomorphism counts by defining a graph join operator $\star$ so that $(F_{v}\star F_{w})$  is obtained by taking the gluing product of $F_{v}$ and $F_{w}$, followed by collapsing $v$ with $w$. For instance, the join of $\FlagGraph[true]{2}{1--2}$ and $\FlagGraph[true]{3}{1--2,2--3,1--3}$ is $\FlagGraph[true]{4}{1--2,2--3,1--3,1--4}$. 
% \begin{lemma}
% For any graphs $G$, $F_{1}$ and $F_{2}$, $\hom(F_{v,1}\star F_{v,2},G_v) = \hom(F_{v,1}, G_v)\hom(F_{v,2}, G_v)$~\cite{Barcelo2021-rs}.
% \end{lemma}
% This indicates that including larger graphs composed of graphs in $\mathcal{F}_v$ does not increase expressivity. Furthermore, given $F$ contains all graphs of size $t$, then we can infer the homomorphism numbers of graphs smaller than $t$.

\begin{lemma}
For any graphs $G$ and $F$, if $|V_F|\leq t \leq |V_G|$, then $\hom(F,G)=\sum_{F':|V_{F'}|=t}a_{F'}\hom(F',G)$ where $a_{F'}\in \mathbb{R}^+$
~\cite{lovasz2012}.
\end{lemma}

We know by now that graph pattern composition does not improve expressivity. And it is unnecessary to include smaller patterns when a complete set of larger graphs of size $t$ is considered. What if we do not have a complete set of patterns of a certain size? Or maybe it is more practical to include small patterns of different sizes. How do we know if any patterns are redundant? Fortunately, we exclude them with linear relations. For a pattern set $\mathcal{F}=\{F_1, \dots, F_m\}$, we define the matrix
$$
\mathbb{M}_{\hom}^{\mathcal{F}}=(\hom(F_i,F_j))^m_{i,j=1}
$$
Clearly, $\mathbb{M}_{\hom}^{\mathcal{F}}$ has a non-zero diagonal (as every pattern has non-zero homomorphism number to itself), but it may be singular, meaning there are linear dependencies.

\[
\begin{blockarray}{lcccccc}
& \FlagGraph{2}{1--2} & \FlagGraph{3}{1--2,2--3} & \FlagGraph{3}{1--2,2--3,1--3} & \FlagGraph{4}{1--2,2--3,3--4} & \FlagGraph{4}{1--2,2--3,1--3,3--4} & \FlagGraph{4}{1--2,2--3,3--4,4--1} \\
\begin{block}{l(cccccc)}
  \FlagGraph{2}{1--2} & 2 & 4 & 6 & 6 & 8 & 8 \\
  \FlagGraph{3}{1--2,2--3} & 2 & 6 & 12 & 10 & 18 & 16\\
  \FlagGraph{3}{1--2,2--3,1--3} & 0 & 0 & 6 & 0 & 6 & 0 \\
  \FlagGraph{4}{1--2,2--3,3--4} & 2 & 8 & 24 & 16 & 38 & 32\\
  \FlagGraph{4}{1--2,2--3,1--3,3--4} & 0 & 0 & 12 & 0 & 14 & 0\\
  \FlagGraph{4}{1--2,2--3,3--4,4--1} & 2 & 8 & 18 & 14 & 28 & 28\\
\end{block}
\end{blockarray}
 \]

 The above is an example of $\mathbb{M}_{\hom}^{\mathcal{F}}$ where $\mathcal{F}=\{ \FlagGraph{2}{1--2}, \FlagGraph{3}{1--2,2--3}, \FlagGraph{3}{1--2,2--3,1--3}, \FlagGraph{4}{1--2,2--3,3--4}, \FlagGraph{4}{1--2,2--3,1--3,3--4}, \FlagGraph{4}{1--2,2--3,3--4,4--1}\}$. The matrix is nonsingular meaning there is no linear relations. However, if we reduce $\mathcal{F}$ to $\{ \FlagGraph{3}{1--2,2--3,1--3}, \FlagGraph{4}{1--2,2--3,3--4}, \FlagGraph{4}{1--2,2--3,1--3,3--4}, \FlagGraph{4}{1--2,2--3,3--4,4--1}\}$ or $\{ \FlagGraph{3}{1--2,2--3,1--3}, \FlagGraph{4}{1--2,2--3,3--4}, \FlagGraph{4}{1--2,2--3,3--4,4--1}\}$, the matrix becomes singular, such as
 \[
\begin{blockarray}{lccc}
& \FlagGraph{3}{1--2,2--3,1--3} & \FlagGraph{4}{1--2,2--3,3--4} & \FlagGraph{4}{1--2,2--3,3--4,4--1} \\
\begin{block}{l(ccc)}
  \FlagGraph{3}{1--2,2--3,1--3} & 6 & 0 & 0 \\
  \FlagGraph{4}{1--2,2--3,3--4} & 24 & 16 & 32\\
  \FlagGraph{4}{1--2,2--3,3--4,4--1} & 18 & 14 & 28\\
\end{block}
\end{blockarray}
 \]
 which has the rank of 2 and has the same distinguishing power as the set $\{ \FlagGraph{3}{1--2,2--3,1--3}, \FlagGraph{4}{1--2,2--3,3--4}\}$
  \[
\begin{blockarray}{lcc}
& \FlagGraph{3}{1--2,2--3,1--3} & \FlagGraph{4}{1--2,2--3,3--4} \\
\begin{block}{l(cc)}
  \FlagGraph{3}{1--2,2--3,1--3} & 6 & 0 \\
  \FlagGraph{4}{1--2,2--3,3--4} & 24 & 16\\
\end{block}
\end{blockarray}
 \]

 In fact, if the nonsingularity of $\mathbb{M}_{\hom}^{\mathcal{F}}$ is retained, adding a graph pattern to $\mathcal{F}$ always improve expressivity.
 \cite{lovasz2012} shows that if $\mathcal{F}$ is a faimily of simple graphs closed under surjective hommomorphism, then $\mathbb{M}_{\hom}^{\mathcal{F}}$ is nonsingular.
 In fact, if $\mathcal{F}$ satisfies this condition, and we further define surjective and injective homomorphism and automorphism in a similar way, denote the corresponding numbers from $F$ as $suj(F,\cdot)$, $inj(F, \cdot)$ and $aut(F)=suj(F,F)=inj(F,F)$, we have $hom(F,G) = \sum_{F'\in\mathcal{F}}\frac{suj(F,F')inj(F',G)}{aut(F)}$. Note $\frac{inj(F',G)}{aut(F)}$ is the matching subgraph number of $F'$ in $G$, so the subgraph numbers can be inferred from homomorphism numbers.

\section{entropy bounds}

Apart from the two cases, commonly, the homomorphism count of a pattern gives some information about the homomorphism count of another pattern. For instance, assuming $\hom(\FlagGraph{2}{1--2}, G)=m$, then we know $m\leq \hom(\FlagGraph{3}{1--2,2--3},G)\leq m^2$. 
$\FlagGraph{3}{1--2,2--3}$ can be surjective-homomorphism mapped to $\FlagGraph{3}{1--2,2--3}$, which gives the lower bound $m$. There are $m$ ways to form a 3-path for each 2-path, giving the upper bound $m^2$.
In fact, the upper bound can be calculated using Shearer's lemma~\cite{shearer1986} to formalize the upper inequality. Let $X_i$ be a random variable, and $\mathrm(H)(X_i)$ be the corresponding entropy.

For example, in \autoref{sec:expressivity}, if $\mathbb{M}_{\hom}^{\mathcal{F}}$ is singular, homomorphism numbers of any two of $\FlagGraph{3}{1--2,2--3,1--3}$, $\FlagGraph{4}{1--2,2--3,3--4}$ and $\FlagGraph{4}{1--2,2--3,3--4,4--1}$ determines the other, so $H(\FlagGraph{3}{1--2,2--3,1--3},  \FlagGraph{4}{1--2,2--3,3--4}, \FlagGraph{4}{1--2,2--3,3--4,4--1}) = H(\FlagGraph{3}{1--2,2--3,1--3},  \FlagGraph{4}{1--2,2--3,3--4}) = H(\FlagGraph{3}{1--2,2--3,1--3}, \FlagGraph{4}{1--2,2--3,3--4,4--1}) = H(\FlagGraph{4}{1--2,2--3,3--4}, \FlagGraph{4}{1--2,2--3,3--4,4--1})$.
Moreover, elements of $\{\hom(F,G)|F\in \mathcal{F}\}$ are not necessarily independent even if $\mathbb{M}_{\hom}^{\mathcal{F}}$ is nonsingular. 
As an example, the conditional entropy $H(\FlagGraph{3}{1--2, 2--3}|\FlagGraph{2}{1--2})$ is smaller than $H(\FlagGraph{3}{1--2,2--3})$ because knowing $\hom(\FlagGraph{2}{1--2}, G)$ gives us information on the lower bound and upper bound of $\hom(\FlagGraph{3}{1--2,2--3}, G)$. In fact, we can use Shearer's lemma to formally bound this relation.

\begin{lemma}
(Shearer's lemma) 
 Let $\mathcal{S}$ be a family of subsets of $[n]=\{1,\dots,n\}$ (possibly with repeats) with each $i \in [n]$ included in at least $t$ members of $\mathcal{S}$. For random vector $(X_1, \dots , X_n)$,
 \begin{equation*}
 \mathrm{H}(X_1,\dots,X_n)\leq\frac{1}{t}\sum_{S\in \mathcal{S}}\mathrm{H}(X_S)
 \end{equation*}
 where $X_S$ is the vector $\{X_i:i\in S\}$
\end{lemma}


\s{There is a formal lower bound using fractional vertex cover \url{https://arxiv.org/pdf/1406.7872.pdf}}

\begin{lemma}
If $\hom(F_1, F_2) \geq 1$ and $|V_{F_1}|\leq |V_{F_2}|$ then there exists a constant $c_1,c_2\in \mathbb{R}^+$ so that 
    \begin{equation*}
    c_1H(F_1)\leq H(F_2)\leq c_2 H(F_1)
    \end{equation*}
\end{lemma}

Apart from the above entropy bound, the gluing product rules related to expressivity in \autoref{sec:expressivity} also apply. Namely, for a gluing product of $F_1$ and $F_2$, $H(F_1F_2)=H(F_1)+H(F_2)$. So including $F_1F_2$ in $\mathcal{F}$ will not increase $H(\mathcal{F})$ if $F_1$ and $F_2$ are already included. However, as we show next, including such glue product in $\mathcal{F}$ increases the generalization bound.



Given $S,\bar{S}\sim \mu_c$, we know
\begin{equation*}
    D_{KL}(\mathbf{X}_{\mathcal{F}\rightarrow S}\| \mathbf{X}_{\mathcal{F}\rightarrow \tilde{S}}) = H(\mathbf{X}_{\mathcal{F}\rightarrow S}, \mathbf{X}_{\mathcal{F}\rightarrow \tilde{S}}) - H(\mathbf{X}_{\mathcal{F}\rightarrow S})
\end{equation*}
We can bound the two entropy using $\mathrm{H}(\mathbf{X}_{\mathcal{F}\rightarrow \mu_c})$.
\begin{align*}
    0 \leq & H(\mathbf{X}_{\mathcal{F}\rightarrow S}, \mathbf{X}_{\mathcal{F}\rightarrow \bar{S}}) \leq 2\mathrm{H}(\mathbf{X}_{\mathcal{F}\rightarrow \mu_c})\\
    0 \leq & H(\mathbf{X}_{\mathcal{F}\rightarrow S}) \leq \mathrm{H}(\mathbf{X}_{\mathcal{F}\rightarrow \mu_c}) \\
    0 \leq & H(\mathbf{X}_{\mathcal{F}\rightarrow \hat{S}}) \leq \mathrm{H}(\mathbf{X}_{\mathcal{F}\rightarrow \mu_c})
\end{align*}
which give a upper bound of the KL divergence.
Combing \cref{thm:wassertein_tv,lemma:tv_dkl,lemma:chuang_bound}, we obtain the result of \cref{lemma:graph_class_bound}.
For each $c\sim p$, it is easy to see $\mathbf{X}_{\mathcal{F}\rightarrow \mu_c} \leq \mathbf{X}_{\mathcal{F}\rightarrow \mu}$. We obtain the result of \cref{lemma:non_class_bound}.
